Shear, pure and simple

In a 2012 article in the International Journal of Non-Linear Mechanics, Destrade et al. showed that for nonlinear elastic materials satisfying Truesdell's so-called empirical inequalities, the deformation corresponding to a Cauchy pure shear stress is not a simple shear. Similar results can be found in a 2011 article of L. A. Mihai and A. Goriely. We confirm their results under weakened assumptions and consider the case of a shear load, i.e. a Biot pure shear stress. In addition, conditions under which Cauchy pure shear stresses correspond to (idealized) pure shear stretch tensors are stated and a new notion of idealized finite simple shear is introduced, showing that for certain classes of nonlinear materials, the results by Destrade et al. can be simplified considerably.

==> tikz/deformationLibrary.tex <==
%TODO : self intersection (shorten grid lines)
%\begin{tikzpicture}[scale = 1.5]
	\newcommand\OmegaSetDefaults{
		\OmegaSetGridSize{.1}{.1}
		\OmegaSetOutlineSampleCount{25}
		\OmegaSetGridSampleCount{5}
		\OmegaSetOutlineToUnitCircle
		\OmegaSetDeformationToId
		\OmegaSetOutlineStyle{thick, color=black}
		\OmegaSetShadingStyle{left color = lightgray, right color = black, opacity = .3}
		\OmegaSetGridStyle{help lines}
		\OmegaSetSmoothOutline
	}
	\newcommand{\OmegaSetOutlineStyle}[1]{
		\tikzset{outlinestyle/.style={#1}}
	}
	\newcommand{\OmegaSetShadingStyle}[1]{
		\tikzset{shadingstyle/.style={#1}}
	}
	\newcommand{\OmegaSetGridStyle}[1]{
		\tikzset{gridstyle/.style={#1}}
	}
	\newcommand{\OmegaSetSharpOutline}{
		\tikzset{outlineplotstyle/.style={sharp plot}}
	}
	\newcommand{\OmegaSetSmoothOutline}{
		\tikzset{outlineplotstyle/.style={smooth}}
	}
	\newcommand{\OmegaSetOutline}[3]{
		\pgfmathdeclarefunction*{omegagammax}{1}{\pgfmathparse{#1(##1)}}
		\pgfmathdeclarefunction*{omegagammay}{1}{\pgfmathparse{#2(##1)}}
		\pgfmathsetmacro{\OmegaParameterlength}{#3}
	}
	\newcommand{\OmegaSetDeformation}[2]{
		\pgfmathdeclarefunction*{omegaphix}{2}{\pgfmathparse{#1(##1, ##2)}}
		\pgfmathdeclarefunction*{omegaphiy}{2}{\pgfmathparse{#2(##1, ##2)}}
	}
	\newcommand{\OmegaSetGridSize}[2]{
		\pgfmathsetmacro{\OmegaGridx}{#1}
		\pgfmathsetmacro{\OmegaGridy}{#2}
	}
	\newcommand{\OmegaSetOutlineSampleCount}[1]{
		\pgfmathsetmacro{\OmegaOutlineSampleCount}{#1}
	}
	\newcommand{\OmegaSetGridSampleCount}[1]{
		\pgfmathsetmacro{\OmegaGridSampleCount}{#1}
	}
	\newcommand{\OmegaSetOutlineToCircle}[3]{
		\pgfmathdeclarefunction*{circx}{1}{\pgfmathparse{#1 + #3*cos(##1)}}
		\pgfmathdeclarefunction*{circy}{1}{\pgfmathparse{#2 + #3*sin(##1)}}
		\OmegaSetOutline{circx}{circy}{360}
	}
	\newcommand{\OmegaSetOutlineToUnitCircle}{
		\OmegaSetOutlineToCircle{0}{0}{1}
	}
	\newcommand{\OmegaSetOutlineToEllipse}[5]{
		\pgfmathdeclarefunction*{ellx}{1}{\pgfmathparse{#1 + #3*cos(##1)*cos(#5) - #4*sin(##1)*sin(#5)}}
		\pgfmathdeclarefunction*{elly}{1}{\pgfmathparse{#2 + #3*cos(##1)*sin(#5) + #4*sin(##1)*cos(#5)}}
		\OmegaSetOutline{ellx}{elly}{360}
	}
	\newcommand{\OmegaSetOutlineToRectangle}[4]{
		\pgfmathsetmacro{\rectWidth}{#3-#1}
		\pgfmathsetmacro{\rectHeight}{#4-#2}
		\pgfmathdeclarefunction*{rectx}{1}{\pgfmathparse{%
			##1<=\rectWidth ? (#1+##1) : (##1<=\rectWidth+\rectHeight ? (#1+\rectWidth) : (##1<=(2*\rectWidth)+\rectHeight ? (#1+\rectWidth-(##1-(\rectWidth+\rectHeight))) : (#1))}%
		}
		\pgfmathdeclarefunction*{recty}{1}{\pgfmathparse{%
			##1<=\rectWidth ? (#2) : (##1<=\rectWidth+\rectHeight ? (#2+##1-\rectWidth) : (##1<=(2*\rectWidth)+\rectHeight ? (#2+\rectHeight) : (#2+\rectHeight-(##1-(2*\rectWidth+\rectHeight)))))}%
		}
		\OmegaSetOutline{rectx}{recty}{2*\rectWidth+2*\rectHeight}
	}
	\newcommand{\OmegaSetDeformationToId}{
		\pgfmathdeclarefunction*{idx}{2}{\pgfmathparse{##1}}
		\pgfmathdeclarefunction*{idy}{2}{\pgfmathparse{##2}}
		\OmegaSetDeformation{idx}{idy}
	}
	\newcommand{\OmegaSetDeformationToSimple}[5]{	% (centerx, centery, weightx, weighty, exponent)
		%(t,y) -> (t-(y-.5)^2/5, y+(t-1)^2/5)
		\pgfmathdeclarefunction*{simplephix}{2}{%
			\pgfmathparse{##1+#3*(##2-#2)^#5}%
		}
		\pgfmathdeclarefunction*{simplephiy}{2}{%
			\pgfmathparse{##2+#4*(##1-#1)^#5}%
		}
		\OmegaSetDeformation{simplephix}{simplephiy}
	}
	\newcommand{\OmegaDraw}{
		\OmegaDrawCustomDeformation{omegaphix}{omegaphiy}
	}
	\newcommand{\OmegaDrawCustomDeformation}[2]{
		\OmegaDrawFull{\OmegaGridx}{\OmegaGridy}{\OmegaParameterlength}{omegagammax}{omegagammay}{#1}{#2}{\OmegaOutlineSampleCount}{\OmegaGridSampleCount}
	}
	\newcommand{\OmegaDrawFull}[9]{	% (#1=gridx, #2=gridy, #3=parameterlength, #4=gammax, #5=gammy,#6= phix, #7=phiy, #8=bordersamples, #9=gridsamples)
		\begin{scope}
			% constants
			\def\conversionFromBoundingBoxUnit{0.03514598035}
			% variables
			\tikzset{borderdomainstyle/.style={domain=0:#3, variable=\t, samples=#8}}
			\tikzset{griddomainstyle/.style={smooth, variable=\t, samples=#9}}
			\newdimen\leftBoundWrongUnit
			\newdimen\rightBoundWrongUnit
			\newdimen\lowerBoundWrongUnit
			\newdimen\upperBoundWrongUnit


			%draw shaded area
			\shade[shadingstyle]
				plot[borderdomainstyle, outlineplotstyle] ({#6(#4(\t), #5(\t))}, {#7(#4(\t), #5(\t))});


			% calculate grid bounds
			\begin{scope}
				% save old bounding box to restore it later (outside the scope)
				\coordinate (oldLowerLeftBound) at (current bounding box.south west);
				\coordinate (oldUpperRightBound) at (current bounding box.north east);

				% create new bounding box
				\pgfresetboundingbox
				\path[use as bounding box]	% undeformed area
					plot[borderdomainstyle, outlineplotstyle] ({#4(\t)}, {#5(\t))});
				\coordinate (lowerLeftBound) at (current bounding box.south west);
				\coordinate (upperRightBound) at (current bounding box.north east);
			\end{scope}
			\pgfextractx{\leftBoundWrongUnit}{\pgfpointanchor{lowerLeftBound}{center}}
			\pgfextractx{\rightBoundWrongUnit}{\pgfpointanchor{upperRightBound}{center}}
			\pgfextracty{\lowerBoundWrongUnit}{\pgfpointanchor{lowerLeftBound}{center}}
			\pgfextracty{\upperBoundWrongUnit}{\pgfpointanchor{upperRightBound}{center}}
			\pgfmathsetmacro{\leftBound}{\conversionFromBoundingBoxUnit*\leftBoundWrongUnit}
			\pgfmathsetmacro{\rightBound}{\conversionFromBoundingBoxUnit*\rightBoundWrongUnit}
			\pgfmathsetmacro{\lowerBound}{\conversionFromBoundingBoxUnit*\lowerBoundWrongUnit}
			\pgfmathsetmacro{\upperBound}{\conversionFromBoundingBoxUnit*\upperBoundWrongUnit}

			% draw grid
			\begin{scope}
				\clip
					plot[borderdomainstyle, outlineplotstyle] ({#6(#4(\t), #5(\t))}, {#7(#4(\t), #5(\t))});

				% draw horizontal lines
				\pgfmathsetmacro{\horizontalGridCount}{(\upperBound-\lowerBound)/#2}
				\foreach \b in {1,2,...,{\horizontalGridCount}}{
					\draw[gridstyle]
						plot[griddomainstyle, domain=\leftBound:\rightBound] ({#6(\t,{\lowerBound+(#2*\b)})},{#7(\t,{\lowerBound+(#2*\b})});
				}

				% draw vertical lines
				\pgfmathsetmacro{\verticalGridCount}{(\rightBound-\leftBound)/#1}
				\foreach \b in {1,2,...,{\verticalGridCount}}{
					\draw[gridstyle]
						plot[griddomainstyle, domain=\lowerBound:\upperBound] ({#6({\leftBound+(#1*\b)},\t)},{#7({\leftBound+(#1*\b)},\t)});
				}
			\end{scope}

			% draw outline
			\draw[outlinestyle]
					plot[borderdomainstyle, outlineplotstyle] ({#6(#4(\t), #5(\t))}, {#7(#4(\t), #5(\t))});

			% restore old bounding box
			\path[use as bounding box] (oldLowerLeftBound) rectangle (oldUpperRightBound);
		\end{scope}
	}

% 	\begin{scope} % global scope for deformation functions
% 		[declare function={
% 			aphix(\x,\y) = \x-(\y-.5)^2/5;
% 			aphiy(\x,\y) = \y+(\x-1)^2/2);
% 			pix(\x,\y) = \x;
% 			piy(\x,\y) = \y;
% 		}]
% 		%\OmegaSetOutline{1.5*sin}{cos}{360}
% 		%\OmegaSetOutlineToCircle{0}{0}{1}
% 		%\OmegaSetOutlineToUnitCircle{0}{0}{1}
% 		%\OmegaSetDeformation{aphix}{aphiy}
% 		\OmegaSetDeformationToId
% 		\OmegaSetOutlineToEllipse{0}{0}{1.75}{1}{45}
% 		\OmegaSetGridSize{.2}{.2}
% 		\OmegaSetGridSampleCount{10}
% 		\OmegaSetOutlineSampleCount{20}
% 		%\OmegaSetOutlineToRectangle{0.0}{0.0}{1.0}{1.0}
% 		\OmegaDraw;
% 		%\OmegaDrawFull{.2}{.2}{360}{sin}{cos}{aphix}{aphiy}
% 	\end{scope}
%\end{tikzpicture}

% DEBUG
%\node at ({gammax(100)},1){\pgfmathparse{gammax(100)}\pgfmathresult};

==> tikz/tikz_PolarDecompositionFiniteSimpleShear.tex <==
\input{tikz/deformationLibrary.tex}

\OmegaSetDefaults
\OmegaSetGridSize{.4}{.4}
\OmegaSetOutlineSampleCount{5}
\OmegaSetGridSampleCount{5}
\OmegaSetOutlineStyle{thick, color=black}
\OmegaSetShadingStyle{left color = lightgray, right color = black, opacity = .0}
\OmegaSetGridStyle{help lines}
\OmegaSetOutlineToRectangle{0}{0}{2}{2}
%\OmegaSetOutlineToUnitCircle

\OmegaSetDeformationToId
\OmegaSetSharpOutline
%\OmegaSetSmoothOutline
%\OmegaDraw

\definecolor{darkgreen}{rgb}{0.15,0.5,0.15}
\definecolor{darkred}{rgb}{1,0.15,0.15}


\def\a{0.4}
\begin{scope}[declare function={
        deformPx(\x,\y)=cosh(\a)*\x+sinh(\a)*\y;
        deformPy(\x,\y)=sinh(\a)*\x+cosh(\a)*\y;
        deformRx(\x,\y)=(cosh(\a)*\x+sinh(\a)*\y)/sqrt(cosh(2*\a));
        deformRy(\x,\y)=(-sinh(\a)*\x+cosh(\a)*\y)/sqrt(cosh(2*\a));
		deformPRx(\x,\y)=deformPx(deformRx(\x,\y),deformRy(\x,\y));
		deformPRy(\x,\y)=deformPy(deformRx(\x,\y),deformRy(\x,\y));
		deformRPx(\x,\y)=deformRx(deformPx(\x,\y),deformPy(\x,\y));
		deformRPy(\x,\y)=deformRy(deformPx(\x,\y),deformPy(\x,\y));
 	}]


	\begin{scope}[xshift=0, yshift=0]

		\begin{scope}[xshift=0, yshift=0]
			\OmegaDraw
			\draw[blue,dashed] (1,0) arc (0:0-atan(tanh(\a)):1);
			\draw[blue,dashed] ({0.9*cos(atan(tanh(\a)))}, {-0.9*sin(atan(tanh(\a)))}) -- ({1.1*cos(atan(tanh(\a)))}, {-1.1*sin(atan(tanh(\a)))});
			\coordinate (a1) at (2.3,1.5);
		\end{scope}

		\begin{scope}[xshift=140, yshift=0]
			\draw[lightgray,dashed] (0,0) -- (2,0) -- (2,2) -- (0,2) -- (0,0);
	    		\OmegaSetDeformation{deformRx}{deformRy}
			\OmegaDraw
	  		\draw[blue,thick,->] (1,0) arc (0:0-atan(tanh(\a)):1);
	  		\draw[blue,thick] (0.9,0) -- (1.1,0);
			%  \draw[blue,dashed] (0,0) -- (0,2);
			%\draw[blue,dashed] (0,1) arc (90:90-atan(tanh(\a)):1);
			\draw[-|,dashed,darkgreen] (0,0) -- (2,2);
			\draw[|-|,dashed,darkgreen] (-1,1) -- (1,-1);  

			\coordinate (a2) at (-0.2,1.5);
			\coordinate (a3) at (2.8,1.5);

		\end{scope}

		\begin{scope}[xshift=280, yshift=0]
			\draw[lightgray,dashed] (0,0) -- ({deformRx(2,0)},{deformRy(2,0)}) -- ({deformRx(2,2)},{deformRy(2,2)}) -- ({deformRx(0,2)},{deformRy(0,2)}) -- (0,0);
	
	    		\OmegaSetDeformation{deformPRx}{deformPRy}
			\OmegaDraw
	  		\draw[darkred] (0,0) -- (0,2);
%			\draw[darkred] (0,1) arc  (90:90-atan(tanh(2*\a)):1) node[pos=0.35,below] {$\scriptsize\vartheta_l$};
			\draw[darkred] (0,2) -- ({2*tanh(2*\a)},2) node[pos=0.5,above] {$\gamma_l$};
			\draw[-|,dashed,darkgreen] (0,0) -- (2,2);
			\draw[|-|,dashed,darkgreen] (-1,1) -- (1,-1);  
			\draw[->,darkgreen] (0,0) -- ({deformPx(2,2)},{deformPy(2,2)});
			\draw[>-<,darkgreen]  ({deformPx(-1,1)},{deformPy(-1,1)}) -- ({deformPx(1,-1)},{deformPy(1,-1)});

			\coordinate (a4) at (-0.2,1.5);

		\end{scope}
		\draw[->,thick] (a1) -- (a2) node[pos=0.5, above] {\large $R$};
		\draw[->,thick] (a3) -- (a4) node[pos=0.5, above] {\large $\sqrt P$};
	
	\end{scope}

	\begin{scope}[xshift=0, yshift=-140]

		\begin{scope}[xshift=0, yshift=0]
			\OmegaDraw
			\draw[-|,dashed,darkgreen] (0,0) -- (2,2);
			\draw[|-|,dashed,darkgreen] (-1,1) -- (1,-1);  
			\coordinate (b1) at (2.3,1.5);
		\end{scope}

		\begin{scope}[xshift=140, yshift=0]
			\draw[lightgray,dashed] (0,0) -- (2,0) -- (2,2) -- (0,2) -- (0,0);

			\OmegaSetDeformation{deformPx}{deformPy}
			\OmegaDraw
			%\draw[<->,thick] (0,0) -- ({deformPx(2,2)},{deformPy(2,2)});
			%\draw[>-<,thick]  ({deformPx(0,2)},{deformPy(0,2)}) -- ({deformPx(2,0)},{deformPy(2,0)});
			\draw[-|,dashed,darkgreen] (0,0) -- (2,2);
			\draw[|-|,dashed,darkgreen] (-1,1) -- (1,-1);  
			\draw[->,darkgreen] (0,0) -- ({deformPx(2,2)},{deformPy(2,2)});
			\draw[>-<,darkgreen]  ({deformPx(-1,1)},{deformPy(-1,1)}) -- ({deformPx(1,-1)},{deformPy(1,-1)});

			%  \draw[blue,dashed] (0,0) -- (0,2);
			%\draw[blue,dashed] (0,1) arc (90:90-atan(tanh(\a)):1);
			\draw[blue,dashed] ({cos(atan(tanh(\a)))}, {sin(atan(tanh(\a)))}) arc (atan(tanh(\a)):0:1);
			\draw[blue,dashed] (0.9,0) -- (1.1,0);

			\coordinate (b2) at (-0.2,1.5);
			\coordinate (b3) at (2.8,1.5);
		\end{scope}

		\begin{scope}[xshift=280, yshift=0]
			\draw[lightgray,dashed] (0,0) -- ({deformPx(2,0)},{deformPy(2,0)}) -- ({deformPx(2,2)},{deformPy(2,2)}) -- ({deformPx(0,2)},{deformPy(0,2)}) -- (0,0);

			\OmegaSetDeformation{deformRPx}{deformRPy}
			\OmegaDraw
			\draw[darkred] (0,0) -- (0,2);
			\draw[darkred] (0,2) -- ({2*sinh(2*\a)},2) node[pos=0.4,above] {$\gamma_r$} -- ({deformRPx(0,2)},{deformRPy(0,2)});

%			\draw[darkred] (0,1) arc (90:90-atan(sinh(2*\a)):1)  node[pos=0.4,below] {$\scriptsize\vartheta_r$};
			\draw[blue,thick,->] ({cos(atan(tanh(\a)))}, {sin(atan(tanh(\a)))}) arc (atan(tanh(\a)):0:1);
			\draw[blue,thick] ({0.9*cos(atan(tanh(\a)))}, {0.9*sin(atan(tanh(\a)))}) -- ({1.1*cos(atan(tanh(\a)))}, {1.1*sin(atan(tanh(\a)))});


			\coordinate (b4) at (-0.2,1.5);
		\end{scope}

		\draw[->,thick] (b1) -- (b2) node[pos=0.5, above] {\large $\sqrt P$};
		\draw[->,thick] (b3) -- (b4) node[pos=0.5, above] {\large $R$};

	\end{scope}


%\draw[->,thick] (-2.4,1.5) .. controls (-0.6,2.2) and (0.6,2.2) ..  (2.4,1.5) node[pos=0.5, above] {\large $F$};
\end{scope}

==> tikz/tikz_functions.tex <==
% styles and functions functions for drawing different deformations and stresses in TikZ
%
%
% styles
\tikzset{bodyStyle/.style={color=black, very thick}}
\tikzset{stressStyle/.style={->, very thick}}
%
% constants
\newcommand{\tikzDefaultArrowDist}{0.2}
\newcommand{\tikzArrowHeadSize}{.14}
%
%
% functions
\newcommand*{\drawDeformation}[4]{ % draw the unit square, deformed by the matrix (#1&#2\\ #3&#4)
	\draw[bodyStyle] (0,0) -- ({#1},{#3}) -- ({(#1)+(#2)},{(#3)+(#4)}) -- ({#2},{#4}) -- cycle;
}
%
\newcommand*{\drawStress}[4]{ % draw the (undeformed) unit square and stress arrows for the stress (#1&#2\\ #3&#4)
	% bounding box (large enough to contain arrow heads)
	\useasboundingbox ({-\tikzDefaultArrowDist-\tikzArrowHeadSize},{-\tikzDefaultArrowDist-\tikzArrowHeadSize}) -- %
		({1+\tikzDefaultArrowDist+\tikzArrowHeadSize},{1+\tikzDefaultArrowDist+\tikzArrowHeadSize});
	% unit square
	\draw[bodyStyle] (0,0) -- (1,0) -- (1,1) -- (0,1) -- cycle;
	% stress arrows
	\draw[stressStyle] (0.5,{1+\tikzDefaultArrowDist}) -- ({0.5+#2},{1+\tikzDefaultArrowDist+#4}); % top arrow
	\draw[stressStyle] (0.5,{-\tikzDefaultArrowDist}) -- ({0.5-#2},{-\tikzDefaultArrowDist-#4}); % bottom arrow
	\draw[stressStyle] ({-\tikzDefaultArrowDist},0.5) -- ({-\tikzDefaultArrowDist-#1},{0.5-#3}); % left arrow
	\draw[stressStyle] ({1+\tikzDefaultArrowDist},0.5) -- ({1+\tikzDefaultArrowDist+#1},{0.5+#3}); % right arrow
}
%
\newcommand*{\drawStressOffset}[8]{ % draw the (undeformed) unit square and stress arrows for the stress (#1&#2\\ #3&#4) with clockwise offsets #5-#8, starting from the top
	% bounding box (large enough to contain arrow heads)
	\useasboundingbox ({-\tikzDefaultArrowDist-\tikzArrowHeadSize},{-\tikzDefaultArrowDist-\tikzArrowHeadSize}) -- %
		({1+\tikzDefaultArrowDist+\tikzArrowHeadSize},{1+\tikzDefaultArrowDist+\tikzArrowHeadSize});
	% unit square
	\draw[bodyStyle] (0,0) -- (1,0) -- (1,1) -- (0,1) -- cycle;
	% stress arrows
	\draw[stressStyle] (0.5,{1+#5}) -- ({0.5+#2},{1+#5+#4}); % top arrow
	\draw[stressStyle] (0.5,{-#7}) -- ({0.5-#2},{-#7-#4}); % bottom arrow
	\draw[stressStyle] ({-#8},0.5) -- ({-#8-#1},{0.5-#3}); % left arrow
	\draw[stressStyle] ({1+#6},0.5) -- ({1+#6+#1},{0.5+#3}); % right arrow
}

==> tikz/tikz_linearPureShearStretch.tex <==
\begin{scope}[x  = {(1cm,0cm)},
                    y  = {(0cm,1cm)},
                    z  = {(0.5cm,0.5cm)},
                    scale = 1]
% style of faces
\definecolor{lightgray2}{rgb}{0.95,0.95,0.95}
\tikzset{facestyle/.style={fill=lightgray2,draw=black,thick,line join=round,opacity=0.65}}
% face "back" 
\def\a{0.3}
\def\gam{0.35}

\begin{scope}[canvas is xy plane at z=0]
  \coordinate (a1) at (0,0);
  \coordinate (a2) at (2,0);
  \coordinate (a3) at (2,2);
  \coordinate (a4) at (0,2);

  \coordinate (a5) at ({5+0},0);
  \coordinate (a6) at ({5+2},{0+\gam});
  \coordinate (a7) at ({5+2+\gam},{2+\gam});
  \coordinate (a8) at ({5+0+\gam},{2});

  \coordinate (ag) at ({5+2},{0});
  \coordinate (ah) at ({5},{2});

\end{scope}
\begin{scope}[canvas is xy plane at z=2]
  \coordinate (b1) at (0,0);
  \coordinate (b2) at (2,0);
  \coordinate (b3) at (2,2);
  \coordinate (b4) at (0,2);

  \coordinate (b5) at ({5+0},0);
  \coordinate (b6) at ({5+2},{0+\gam});
  \coordinate (b7) at ({5+2+\gam},{2+\gam});
  \coordinate (b8) at ({5+0+\gam},{2});
\end{scope}

\begin{scope}[canvas is xy plane at z=1]
  \coordinate (c1) at (1.5,2.4);
  \coordinate (c2) at (4,3.5);
  \coordinate (c3) at ({5.1+\gam/2+1},{0.2+2+\gam/2});
\end{scope}

\path[facestyle] (b1) -- (b2) -- (b3) -- (b4) -- (b1);%hinten
\path[facestyle] (a1) -- (a2) -- (b2) -- (b1) -- (a1);%unten
\path[facestyle] (a1) -- (b1) -- (b4) -- (a4) -- (a1);%links
\path[facestyle] (a4) -- (a3) -- (b3) -- (b4) -- (a4) node[pos=0.4, left=0.2em] {1};%oben
\path[facestyle] (a2) -- (b2) -- (b3) -- (a3) -- (a2);%rechts
\path[facestyle] (a1) -- (a2)  node[pos=0.5, below] {1} -- (a3) -- (a4) -- (a1) node[pos=0.5, left] {1} ;%vorne

\path[facestyle] (b5) -- (b6) -- (b7) -- (b8) -- (b5);%hinten
\path[facestyle] (a5) -- (a6) -- (b6) -- (b5) -- (a5);%unten
\path[facestyle] (a5) -- (b5) -- (b8) -- (a8) -- (a5);%links
\path[facestyle] (a8) -- (a7) -- (b7) -- (b8) -- (a8) node[pos=0.4, left=0.2em] {1};%oben
\path[facestyle] (a6) -- (b6) -- (b7) -- (a7) -- (a6);%rechts
\path[facestyle] (a5) -- (a6)  -- (a7) -- (a8) -- (a5);%vorne

\path[draw=black] (a5) -- (ag) node[pos=0.50,below=-0.2em] {\tiny$\underbrace{\hspace{8.3em}}_{1}$} -- (a6) node[pos=0.51, right=-0.3em] {\tiny$\left.\begin{matrix}\\[0.5em]\end{matrix}\right\}\frac\gamma2$};
%\path[draw=black] (a6) -- (a7) -- (ag) node[pos=0.51, right=-0.3em] {\tiny$\left.\begin{matrix}\\[8.7em]\end{matrix}\right\}\sqrt{\cosh(2\alpha)}$} -- (a6) node[pos=0.49,below=-0.2em] {\tiny$\underbrace{\hspace{5.5em}}_\frac{\sinh(2\alpha)}{\sqrt{\cosh(2\alpha)}}$};

\draw[->,thick] (c1) .. controls (c2) .. (c3) node[pos=0.5, above] {\large $P$};

%\path[draw=black] (a5) -- (ah);
%\draw (a5) pic{carc=-30:30:2em} ;
%\draw (a5) ++(90:1.2) arc (90:{90-atan(tanh(\a))}:1.2) node[left=-0.1em]{$\overset{\phantom b}{\vartheta}$};
\end{scope}


==> tikz/tikz_plotBiotShearVL.tex <==
\begin{scope}[scale=1, trim axis left, trim axis right]
	\pgfplotsset{axisStyle/.style={axis x line=middle, axis y line=middle}}
	\tikzset{zoomedInGraphStyle/.style={smooth, color=blue, thick}}
	\tikzset{defaultGraphStyle/.style={smooth, color=red, thick}}

	\begin{scope}
		\begin{axis}[axisStyle,xmin=0, ymax=4.2]
			\addplot[zoomedInGraphStyle, samples=100, domain=.049:1] {2*(x-ln(x)-1)};
			\addplot[zoomedInGraphStyle, samples=100, domain=1:3.024] {(x-1)^2} node[pos=.5, above left]{$\widehat{w}$};
			\addplot[zoomedInGraphStyle, color=red, samples=100, domain=.0007:3.36] {x*(ln(x)-1)+1} node[pos=.77, below right]{$\widetilde{w}$};
		\end{axis}
	\end{scope}
\end{scope}

==> tikz/tikz_pureShearDeformation.tex <==
\input{tikz/tikz_functions.tex}
\drawDeformation{sqrt(5.0)/2.0}{.5}{.5}{sqrt(5.0)/2.0};

==> tikz/tikz_pureShearDeformationDiagonal.tex <==
\input{tikz/tikz_functions.tex}
\drawDeformation{1.5}{0}{0}{2.0/3.0};

==> tikz/tikz_pureShearStress.tex <==
\input{tikz/tikz_functions.tex}
\drawStress{0}{.5}{.5}{0};

==> tikz/tikz_pureShearStressDiagonal.tex <==
\input{tikz/tikz_functions.tex}
\drawStressOffset{.5}{0}{0}{-.5}{.6}{.1}{.6}{.1};

==> tikz/tikz_pureShearStressSimpleShear.tex <==
\input{\tikzpath/deformationLibrary.tex}

\OmegaSetDefaults
\OmegaSetGridSize{.4}{.4}
\OmegaSetOutlineSampleCount{5}
\OmegaSetGridSampleCount{5}
\OmegaSetOutlineStyle{thick, color=black}
\OmegaSetShadingStyle{left color = lightgray, right color = black, opacity = .0}
\OmegaSetGridStyle{help lines}
\OmegaSetOutlineToRectangle{0}{0}{2}{2}
%\OmegaSetOutlineToUnitCircle

\OmegaSetDeformationToId
\OmegaSetSharpOutline
%\OmegaSetSmoothOutline
%\OmegaDraw

\definecolor{darkred}{rgb}{1,0.15,0.15}
\definecolor{darkgreen}{rgb}{0.15,0.5,0.15}
\definecolor{darkblue}{rgb}{0.15,0.15,0.5}


\definecolor{lightgray2}{rgb}{0.95,0.95,0.95}
\tikzset{facestyle/.style={fill=lightgray2,draw=black,thick,line join=round,opacity=0.65}}


\def\gam{0.4}
\def\s{0.5}

\begin{scope}[declare function={
        deformFx(\x,\y,\g)=\x+\g*\y;
        deformFy(\x,\y,\g)=\y;
        deformCofFx(\x,\y,\g)=\x;
        deformCofFy(\x,\y,\g)=-\g*\x+\y;
		deformRx(\x,\y,\g)=2/sqrt(4+\g^2)*\x + \g/sqrt(4+\g^2)*\y;
		deformRy(\x,\y,\g)=-\g/sqrt(4+\g^2)*\x + 2/sqrt(4+\g^2)*\y;
		deformRtx(\x,\y,\g)=2/sqrt(4+\g^2)*\x - \g/sqrt(4+\g^2)*\y;
		deformRty(\x,\y,\g)=\g/sqrt(4+\g^2)*\x + 2/sqrt(4+\g^2)*\y;
 	}]

	\begin{scope}[xshift=0, yshift=0] %cauchy
	
		\begin{scope}[xshift=0, yshift=0]

			\begin{scope}[canvas is xy plane at z=0]
				  \coordinate (a1) at (0,0);
				  \coordinate (a2) at (2,0);
				  \coordinate (a3) at (2,2);
				  \coordinate (a4) at (0,2);
			\end{scope}

			\begin{scope}[canvas is xy plane at z=2]
				  \coordinate (a5) at (0,0);
				  \coordinate (a6) at (2,0);
				  \coordinate (a7) at (2,2);
				  \coordinate (a8) at (0,2);
			\end{scope}

			\begin{scope}[canvas is xy plane at z=1]
				  \coordinate (p1) at (2,1);
				  \coordinate (p2) at (1,2);
				  \coordinate (p3) at (0,1);
				  \coordinate (p4) at (1,0);

				  \coordinate (p1e) at ({2+deformRtx(\s*deformCofFy(1,0,\gam),\s*deformCofFx(1,0,\gam),\gam)},{1+deformRty(\s*deformCofFy(1,0,\gam),\s*deformCofFx(1,0,\gam),\gam)});
				  \coordinate (p2e) at ({1+deformRtx(\s*deformCofFy(0,1,\gam),\s*deformCofFx(0,1,\gam),\gam)},{2+deformRty(\s*deformCofFy(0,1,\gam),\s*deformCofFx(0,1,\gam),\gam)});
				  \coordinate (p3e) at ({0+deformRtx(\s*deformCofFy(-1,0,\gam),\s*deformCofFx(-1,0,\gam),\gam)},{1+deformRty(\s*deformCofFy(-1,0,\gam),\s*deformCofFx(-1,0,\gam),\gam)});
				  \coordinate (p4e) at ({1+deformRtx(\s*deformCofFy(0,-1,\gam),\s*deformCofFx(0,-1,\gam),\gam)},{0+deformRty(\s*deformCofFy(0,-1,\gam),\s*deformCofFx(0,-1,\gam),\gam)});

				  \coordinate (p1ep) at ({2},{1+deformRty(\s*deformCofFy(1,0,\gam),\s*deformCofFx(1,0,\gam),\gam)});
				  \coordinate (p2ep) at ({1+deformRtx(\s*deformCofFy(0,1,\gam),\s*deformCofFx(0,1,\gam),\gam)},{2});
				  \coordinate (p3ep) at ({0},{1+deformRty(\s*deformCofFy(-1,0,\gam),\s*deformCofFx(-1,0,\gam),\gam)});
				  \coordinate (p4ep) at ({1+deformRtx(\s*deformCofFy(0,-1,\gam),\s*deformCofFx(0,-1,\gam),\gam)},{0});
%				  \coordinate (p1e) at ({2},{1);
%				  \coordinate (p2e) at ({1},{2});
%				  \coordinate (p3e) at ({0},{1});
%				  \coordinate (p4e) at ({1},{0});

				\coordinate (c1) at (3,1);

			\end{scope}

			\path[facestyle] (a1) -- (a2)  -- (a3) -- (a4) -- (a1)  ;%hinten
			\path[facestyle] (a1) -- (a4)  -- (a8) -- (a5) -- (a1)  ;%links
			\path[facestyle] (a1) -- (a2)  -- (a6) -- (a5) -- (a1)  ;%unten

			\draw[->,thick] (p1) -- (p1e);
			\draw[->,thick] (p3) -- (p3e);
			\draw[->,thick] (p4) -- (p4e);

			\draw[dotted] (p1) -- (p1ep);
			\draw[dotted] (p2) -- (p2ep);
			\draw[dotted] (p3) -- (p3ep);
			\draw[dotted] (p4) -- (p4ep);
%			\draw[gray] (p1ep) -- (p1e);

			\path[facestyle] (a4) -- (a3)  -- (a7) -- (a8) -- (a4)  ;%oben
			\path[facestyle] (a2) -- (a3)  -- (a7) -- (a6) -- (a2)  ;%rechts
			\path[facestyle] (a5) -- (a6)  -- (a7) -- (a8) -- (a5)  ;%vorne

			\draw[->,thick] (p2) -- (p2e);
	
		\end{scope}


		\begin{scope}[xshift=150, yshift=0]

			\begin{scope}[canvas is xy plane at z=0]
				  \coordinate (a1) at ({deformFx(0,0,\gam)},{deformFy(0,0,\gam)});
				  \coordinate (a2) at ({deformFx(2,0,\gam)},{deformFy(2,0,\gam)});
				  \coordinate (a3) at ({deformFx(2,2,\gam)},{deformFy(2,2,\gam)});
				  \coordinate (a4) at ({deformFx(0,2,\gam)},{deformFy(0,2,\gam)});
			\end{scope}

			\begin{scope}[canvas is xy plane at z=2]
				\coordinate (a5) at ({deformFx(0,0,\gam)},{deformFy(0,0,\gam)});
				\coordinate (a6) at ({deformFx(2,0,\gam)},{deformFy(2,0,\gam)});
				\coordinate (a7) at ({deformFx(2,2,\gam)},{deformFy(2,2,\gam)});
				\coordinate (a8) at ({deformFx(0,2,\gam)},{deformFy(0,2,\gam)});
			\end{scope}

\def\wuerfelgr{0.6}
\def\wuerfelx{1.3}
\def\wuerfely{1}

			\begin{scope}[canvas is xy plane at z={1-\wuerfelgr/2}]
				  \coordinate (ak1) at ({\wuerfelx-\wuerfelgr/2},{\wuerfely-\wuerfelgr/2});
				  \coordinate (ak2) at ({\wuerfelx+\wuerfelgr/2},{\wuerfely-\wuerfelgr/2});
				  \coordinate (ak3) at ({\wuerfelx+\wuerfelgr/2},{\wuerfely+\wuerfelgr/2});
				  \coordinate (ak4) at ({\wuerfelx-\wuerfelgr/2},{\wuerfely+\wuerfelgr/2});
			\end{scope}

			\begin{scope}[canvas is xy plane at z={1+\wuerfelgr/2}]
				  \coordinate (ak5) at ({\wuerfelx-\wuerfelgr/2},{\wuerfely-\wuerfelgr/2});
				  \coordinate (ak6) at ({\wuerfelx+\wuerfelgr/2},{\wuerfely-\wuerfelgr/2});
				  \coordinate (ak7) at ({\wuerfelx+\wuerfelgr/2},{\wuerfely+\wuerfelgr/2});
				  \coordinate (ak8) at ({\wuerfelx-\wuerfelgr/2},{\wuerfely+\wuerfelgr/2});
			\end{scope}



			\begin{scope}[canvas is xy plane at z=1]
				\coordinate (p1w) at ({\wuerfelx+\wuerfelgr/2},{\wuerfely});
				\coordinate (p1ew) at ({\wuerfelx+\wuerfelgr/2},{\wuerfely+\wuerfelgr/2*0.6});
				\coordinate (p2w) at ({\wuerfelx},{\wuerfely+\wuerfelgr/2});
				\coordinate (p2ew) at ({\wuerfelx+\wuerfelgr/2*0.6},{\wuerfely+\wuerfelgr/2});

				\coordinate (p1) at ({deformFx(2,1,\gam)},{deformFy(2,1,\gam)});
				\coordinate (p2) at ({deformFx(1,2,\gam)},{deformFy(1,2,\gam)});
				\coordinate (p3) at ({deformFx(0,1,\gam)},{deformFy(0,1,\gam)});
				\coordinate (p4) at ({deformFx(1,0,\gam)},{deformFy(1,0,\gam)});

				\coordinate (p1e) at ({deformFx(2,1,\gam)+\s*deformCofFy(1,0,\gam)*sqrt(1+\gam^2)},{deformFy(2,1,\gam)+\s*deformCofFx(1,0,\gam)*sqrt(1+\gam^2)}); %hÃÂ¤ndisch flÃÂ¤chenverzerrung *sqrt(1+\gam^2) hinzugefÃÂ¼gt
				\coordinate (p2e) at ({deformFx(1,2,\gam)+\s*deformCofFy(0,1,\gam)},{deformFy(1,2,\gam)+\s*deformCofFx(0,1,\gam)});
				\coordinate (p3e) at ({deformFx(0,1,\gam)+\s*deformCofFy(-1,0,\gam)*sqrt(1+\gam^2)},{deformFy(0,1,\gam)+\s*deformCofFx(-1,0,\gam)*sqrt(1+\gam^2)});
				\coordinate (p4e) at ({deformFx(1,0,\gam)+\s*deformCofFy(0,-1,\gam)},{deformFy(1,0,\gam)+\s*deformCofFx(0,-1,\gam)});

				\coordinate (p1ep) at ({deformFx(2,1,\gam)+\s*deformCofFy(1,0,\gam)*sqrt(1+\gam^2)},{deformFy(2,1,\gam)+\s*deformCofFx(1,0,\gam)*sqrt(1+\gam^2)}); %hÃÂ¤ndisch flÃÂ¤chenverzerrung *sqrt(1+\gam^2) hinzugefÃÂ¼gt
				\coordinate (p2ep) at ({deformFx(1,2,\gam)+\s*deformCofFy(0,1,\gam)},{deformFy(1,2,\gam)+\s*deformCofFx(0,1,\gam)});
				\coordinate (p3ep) at ({deformFx(0,1,\gam)+\s*deformCofFy(-1,0,\gam)*sqrt(1+\gam^2)},{deformFy(0,1,\gam)+\s*deformCofFx(-1,0,\gam)*sqrt(1+\gam^2)});
				\coordinate (p4ep) at ({deformFx(1,0,\gam)+\s*deformCofFy(0,-1,\gam)},{deformFy(1,0,\gam)+\s*deformCofFx(0,-1,\gam)});

				\coordinate (c2) at (-0.7,1);

			\end{scope}


			\draw[->,thick] (c1) -- (c2) node[pos=0.5,above] {$F$};

			\path[facestyle] (a1) -- (a2)  -- (a3) -- (a4) -- (a1)  ;%hinten
			\path[facestyle] (a1) -- (a4)  -- (a8) -- (a5) -- (a1)  ;%links
			\path[facestyle] (a1) -- (a2)  -- (a6) -- (a5) -- (a1)  ;%unten

			\draw[->,thick] (p1) -- (p1e);
			\draw[->,thick] (p3) -- (p3e);
			\draw[->,thick] (p4) -- (p4e);
			\draw[gray] (p1) -- (p1ep);
			\draw[gray] (p2) -- (p2ep);
			\draw[gray] (p3) -- (p3ep);
			\draw[gray] (p4) -- (p4ep);

			\path[facestyle] (ak4) -- (ak3)  -- (ak7) -- (ak8) -- (ak4)  ;%oben
			\path[facestyle] (ak2) -- (ak3)  -- (ak7) -- (ak6) -- (ak2)  ;%rechts
			\path[facestyle] (ak5) -- (ak6)  -- (ak7) -- (ak8) -- (ak5)  ;%vorne
			\draw[->,line width=0.1mm] (p1w) -- (p1ew);
			\draw[->,line width=0.1mm] (p2w) -- (p2ew);


			\path[facestyle] (a4) -- (a3)  -- (a7) -- (a8) -- (a4)  ;%oben
			\path[facestyle] (a2) -- (a3)  -- (a7) -- (a6) -- (a2)  ;%rechts
			\path[facestyle] (a5) -- (a6)  -- (a7) -- (a8) -- (a5)  ;%vorne

			\draw[->,thick] (p2) -- (p2e);

			\draw[darkblue]  (0.3,-1.4) node {pure shear Cauchy stress};
	
		\end{scope}
	\end{scope}


	\begin{scope}[xshift=0, yshift=-130] %biot
	
		\begin{scope}[xshift=0, yshift=0]

			\begin{scope}[canvas is xy plane at z=0]
				  \coordinate (a1) at (0,0);
				  \coordinate (a2) at (2,0);
				  \coordinate (a3) at (2,2);
				  \coordinate (a4) at (0,2);
			\end{scope}

			\begin{scope}[canvas is xy plane at z=2]
				  \coordinate (a5) at (0,0);
				  \coordinate (a6) at (2,0);
				  \coordinate (a7) at (2,2);
				  \coordinate (a8) at (0,2);
			\end{scope}


			\begin{scope}[canvas is xy plane at z=1]

				\coordinate (p1) at (2,1);
				\coordinate (p2) at (1,2);
				\coordinate (p3) at (0,1);
				\coordinate (p4) at (1,0);

				\coordinate (p1e) at (2,{1+\s});
				\coordinate (p2e) at ({1+\s},2);
				\coordinate (p3e) at (0,{1-\s});
				\coordinate (p4e) at ({1-\s},0);

				\coordinate (c1) at (3,1);

			\end{scope}

			\path[facestyle] (a1) -- (a2)  -- (a3) -- (a4) -- (a1)  ;%hinten
			\path[facestyle] (a1) -- (a4)  -- (a8) -- (a5) -- (a1)  ;%links
			\path[facestyle] (a1) -- (a2)  -- (a6) -- (a5) -- (a1)  ;%unten

			\draw[->,thick] (p3) -- (p3e);
			\draw[->,thick] (p4) -- (p4e);


			\path[facestyle] (a4) -- (a3)  -- (a7) -- (a8) -- (a4)  ;%oben
			\path[facestyle] (a2) -- (a3)  -- (a7) -- (a6) -- (a2)  ;%rechts
			\path[facestyle] (a5) -- (a6)  -- (a7) -- (a8) -- (a5)  ;%vorne

			\draw[->,thick] (p1) -- (p1e);
			\draw[->,thick] (p2) -- (p2e);

			\draw[darkblue]  (0.2,-1.4) node {pure shear Biot stress};
	
		\end{scope}


		\begin{scope}[xshift=150, yshift=0]

			\begin{scope}[canvas is xy plane at z=0]
				  \coordinate (a1) at ({deformFx(0,0,\gam)},{deformFy(0,0,\gam)});
				  \coordinate (a2) at ({deformFx(2,0,\gam)},{deformFy(2,0,\gam)});
				  \coordinate (a3) at ({deformFx(2,2,\gam)},{deformFy(2,2,\gam)});
				  \coordinate (a4) at ({deformFx(0,2,\gam)},{deformFy(0,2,\gam)});
			\end{scope}

			\begin{scope}[canvas is xy plane at z=2]
				\coordinate (a5) at ({deformFx(0,0,\gam)},{deformFy(0,0,\gam)});
				\coordinate (a6) at ({deformFx(2,0,\gam)},{deformFy(2,0,\gam)});
				\coordinate (a7) at ({deformFx(2,2,\gam)},{deformFy(2,2,\gam)});
				\coordinate (a8) at ({deformFx(0,2,\gam)},{deformFy(0,2,\gam)});
			\end{scope}


			\begin{scope}[canvas is xy plane at z=1]
				\coordinate (p1) at ({deformFx(2,1,\gam)},{deformFy(2,1,\gam)});
				\coordinate (p2) at ({deformFx(1,2,\gam)},{deformFy(1,2,\gam)});
				\coordinate (p3) at ({deformFx(0,1,\gam)},{deformFy(0,1,\gam)});
				\coordinate (p4) at ({deformFx(1,0,\gam)},{deformFy(1,0,\gam)});

%\def\gam{0}

				  \coordinate (p1e) at ({deformFx(2,1,\gam)+deformRx(0,\s,\gam)*sqrt(1+\gam^2)},{deformFy(2,1,\gam)+deformRy(0,\s,\gam)*sqrt(1+\gam^2)});
%				  \coordinate (p1e) at ({deformFx(2,1,\gam)+0},{deformFy(2,1,\gam)+\s});
				  \coordinate (p2e) at ({deformFx(1,2,\gam)+deformRx(\s,0,\gam)},{deformFy(1,2,\gam)+deformRy(\s,0,\gam)});
				  \coordinate (p3e) at ({deformFx(0,1,\gam)+deformRx(0,-\s,\gam)*sqrt(1+\gam^2)},{deformFy(0,1,\gam)+deformRy(0,-\s,\gam)*sqrt(1+\gam^2)});
				  \coordinate (p4e) at ({deformFx(1,0,\gam)+deformRx(-\s,0,\gam)},{deformFy(1,0,\gam)+deformRy(-\s,0,\gam)});

%				\coordinate (p1e) at ({deformFx(2,1+\s,\gam)},{deformFy(2,1+\s,\gam)});
%%				\coordinate (p1e) at ({deformFx(2,1)+\g*\s},{deformFy(2,1)+\s});
%				\coordinate (p2e) at ({deformFx(1+\s,2,\gam)},{deformFy(1+\s,2,\gam)});
%				\coordinate (p3e) at ({deformFx(0,1-\s,\gam)},{deformFy(0,1-\s,\gam)});
%				\coordinate (p4e) at ({deformFx(1-\s,0,\gam)},{deformFy(1-\s,0,\gam)});

				\coordinate (c2) at (-0.7,1);

			\end{scope}

			\draw[->,thick] (c1) -- (c2) node[pos=0.5,above] {$F$};

			\path[facestyle] (a1) -- (a2)  -- (a3) -- (a4) -- (a1)  ;%hinten
			\path[facestyle] (a1) -- (a4)  -- (a8) -- (a5) -- (a1)  ;%links
			\path[facestyle] (a1) -- (a2)  -- (a6) -- (a5) -- (a1)  ;%unten

			\draw[->,thick] (p1) -- (p1e);
			\draw[->,thick] (p2) -- (p2e);
			\draw[->,thick] (p3) -- (p3e);
			\draw[->,thick] (p4) -- (p4e);


			\path[facestyle] (a4) -- (a3)  -- (a7) -- (a8) -- (a4)  ;%oben
			\path[facestyle] (a2) -- (a3)  -- (a7) -- (a6) -- (a2)  ;%rechts
			\path[facestyle] (a5) -- (a6)  -- (a7) -- (a8) -- (a5)  ;%vorne

	
		\end{scope}
	\end{scope}




%\draw[->,thick] (-2.4,1.5) .. controls (-0.6,2.2) and (0.6,2.2) ..  (2.4,1.5) node[pos=0.5, above] {\large $F$};
\end{scope}

==> tikz/tikz_simpleFiniteShear.tex <==
\input{tikz/tikz_functions.tex}
\drawDeformation{0.343}{1.286}{0}{1.4577};

==> tikz/tikz_simpleShear.tex <==
\input{tikz/tikz_functions.tex}
\drawDeformation{1}{.5}{0}{1};
